Connect-while-in-range: modelling the impact of spatial constraints on dynamic communication network structures

Like other social animals and biological systems, human groups constantly exchange information. Network models provide a way of quantifying this process by representing the pathways of information propagation between individuals. Existing approaches to studying these networks largely hypothesize network formation to be a result of cognitive biases and choices about who to connect to. Observational data suggests, however, that physical proximity plays a major role in shaping the formation of communication networks in human groups. Here we report results from a series of agent-based simulations in which agents move around at random in a bounded 2D space and connect while within communication range. Comparing the results to a non-spatial model, we show how including spatial constraints impacts our predictions of network structure: ranged networks are more clustered, with slightly higher degree, higher average shortest path length, a lower number of connected components and a higher small-world index. We find two important drivers of network structure in range-constrained dynamic networks: communication range relative to environment size, and population density. These results show that neglecting spatial constraints in models of network formation makes a difference for predicted network structures. Our simulation model quantifies this part of the process of network formation, realized by simply situating individuals in an environment. The model also provides a tool to include spatial constraints in other models of human communication, as well as dynamic models of network formation more generally.

==> References.tex <==
@book{acerbi2020cultural,
  title={Cultural Evolution in the Digital Age},
  author={Acerbi, Alberto},
  year={2020},
  publisher={MIT Press},
  address={Cambridge, MA},
  url={https://mitpress.mit.edu/9780262044712/cultural-evolution-in-the-digital-age/}
}

@article{almaatouqAdaptiveSocialNetworks2020,
  title = {Adaptive Social Networks Promote the Wisdom of Crowds},
  author = {Almaatouq, Abdullah and {Noriega-Campero}, Alejandro and Alotaibi, Abdulrahman and Krafft, P. M. and Moussaid, Mehdi and Pentland, Alex},
  year = {2020},
  month = may,
  journal = {Proceedings of the National Academy of Sciences of the United States of America},
  volume = {117},
  number = {21},
  pages = {11379--11386},
  issn = {1091-6490},
  doi = {10.1073/pnas.1917687117},
  abstract = {Social networks continuously change as new ties are created and existing ones fade. It is widely acknowledged that our social embedding has a substantial impact on what information we receive and how we form beliefs and make decisions. However, most empirical studies on the role of social networks in collective intelligence have overlooked the dynamic nature of social networks and its role in fostering adaptive collective intelligence. Therefore, little is known about how groups of individuals dynamically modify their local connections and, accordingly, the topology of the network of interactions to respond to changing environmental conditions. In this paper, we address this question through a series of behavioral experiments and supporting simulations. Our results reveal that, in the presence of plasticity and feedback, social networks can adapt to biased and changing information environments and produce collective estimates that are more accurate than their best-performing member. To explain these results, we explore two mechanisms: 1) a global-adaptation mechanism where the structural connectivity of the network itself changes such that it amplifies the estimates of high-performing members within the group (i.e., the network "edges" encode the computation); and 2) a local-adaptation mechanism where accurate individuals are more resistant to social influence (i.e., adjustments to the attributes of the "node" in the network); therefore, their initial belief is disproportionately weighted in the collective estimate. Our findings substantiate the role of social-network plasticity and feedback as key adaptive mechanisms for refining individual and collective judgments.},
  langid = {english},
  pmcid = {PMC7260971},
  pmid = {32393632},
  keywords = {collective intelligence,complex adaptive systems,Feedback Psychological,Humans,Intelligence,Judgment,Models Theoretical,Nontherapeutic Human Experimentation,Random Allocation,Social Behavior,Social Networking,social networks,virtual labs,wisdom of crowds},
  file = {C:\Users\niekk\Zotero\storage\LF2KVY8L\Almaatouq et al. - 2020 - Adaptive social networks promote the wisdom of cro.pdf}
}

@inproceedings{almaatouqMobileCommunicationSignatures2016,
  title = {Mobile Communication Signatures of Unemployment},
  author = {Almaatouq, Abdullah and Prieto-Castrillo, Francisco and Pentland, Alex},
  booktitle = {Computational Social Science: Discovery and Prediction},
  editor = {Aiello, Luca Maria and McFarland, Daniel},
  year = {2016},
  month = sep,
  pages = {413--428},
  abstract = {The mapping of populations socio-economic well-being is highly constrained by the logistics of censuses and surveys. Consequently, spatially detailed changes across scales of days, weeks, or months, or even year to year, are difficult to assess; thus the speed of which policies can be designed and evaluated is limited. However, recent studies have shown the value of mobile phone data as an enabling methodology for demographic modeling and measurement. In this work, we investigate whether indicators extracted from mobile phone usage can reveal information about the socio-economical status of microregions such as districts (i.e., average spatial resolution {$<$} 2.7km). For this we examine anonymized mobile phone metadata combined with beneficiaries records from unemployment benefit program. We find that aggregated activity, social, and mobility patterns strongly correlate with unemployment. Furthermore, we construct a simple model to produce accurate reconstruction of district level unemployment from their mobile communication patterns alone. Our results suggest that reliable and cost-effective economical indicators could be built based on passively collected and anonymized mobile phone data. With similar data being collected every day by telecommunication services across the world, survey-based methods of measuring community socioeconomic status could potentially be augmented or replaced by such passive sensing methods in the future.},
  isbn = {978-3-319-47879-1},
  file = {C:/Users/niekk/Zotero/storage/YTJKBHKU/Almaatouq et al. - 2016 - Mobile Communication Signatures of Unemployment.pdf}
}

@article{baldiniRevisitingEffectPopulation,
  title = {Revisiting the Effect of Population Size on Cumulative Cultural Evolution},
  author = {Baldini, Ryan},
  journal = {Journal of Cognition and Culture},
  year = {2015},
  volume = {15},
  number = {1-2},
  pages = {118--139},
  doi = {10.1163/15685373-12342142},
  abstract = {Henrich (2004) argued that larger populations can better maintain complex technologies because they contain more highly skilled people whom others can imitate. His original model, however, did not distinguish the effects of population size from population density or network size; a learner's social network included the entire population. Does population size remain important when populations are subdivided and networks are realistically small? I use a mathematical model to show that population size has little effect on equilibrium levels of mean skill under a wide range of conditions. The effects of network size and transmission error rate usually overshadow that of population size. Population size can, however, affect the rate at which a population approaches equilibrium, by increasing the rate at which innovations arise. This effect is small unless innovation is very rare. Whether population size predicts technological complexity in the real world, then, depends on whether technological evolution is innovation-limited and short of equilibrium. The effect of population ``connectedness,'' via migration or trade, is similar. I discuss the results of this analysis in light of the current empirical debate.},
  langid = {english},
  file = {C:/Users/niekk/Zotero/storage/T86IY5TL/Baldini - Revisiting the effect of population size on cumula.pdf}
}


@article{barabasiScaleFreeCharacteristicsRandom2000,
  title = {Scale-{{Free Characteristics}} of {{Random Networks}}: {{The Topology}} of the {{World-Wide Web}}},
  shorttitle = {Scale-{{Free Characteristics}} of {{Random Networks}}},
  author = {Barabasi, Albert-Laszlo and Albert, R{\'e}ka and Jeong, Hawoong},
  year = {2000},
  month = jun,
  journal = {Physica A: Statistical Mechanics and its Applications},
  volume = {281},
  pages = {69--77},
  doi = {10.1016/S0378-4371(00)00018-2},
  abstract = {The world-wide web forms a large directed graph, whose vertices are documents and edges are links pointing from one document to another. Here we demonstrate that despite its apparent random character, the topology of this graph has a number of universal scale-free characteristics. We introduce a model that leads to a scale-free network, capturing in a minimal fashion the self-organization processes governing the world-wide web. c \# 2000 Elsevier Science B.V. All rights reserved. PACS: 84.35.+i; 64.60.Fr; 87.23.Ge Keywords: Disordered systems; Networks; Random networks; Critical phenomena; Scaling; World-wide web 1. Introduction The emergence of order in natural systems is a constant source of fascination and inspiration for both physical and biological sciences. While the spatial order characterizing for example the crystals has been at the basis of many advances in contemporary physics, most complex systems in nature do not o\#er such high degree of order. In fact, many systems ...},
  file = {C:\Users\niekk\Zotero\storage\HGRXBMZW\Barabasi et al. - 2000 - Scale-Free Characteristics of Random Networks The.pdf}
}

@inproceedings{backstrom2011anatomy,
  title={The anatomy of the Facebook social graph},
  author={Backstrom, Lars and Boldi, Paolo and Rosa, Marco and Ugander, Johan and Vigna, Sebastiano},
  booktitle={Proceedings of the 21st international conference on World Wide Web},
  pages={831--840},
  year={2011},
  organization={ACM}
}

@article{bavelasCommunicationPatternsTask1950,
  title = {Communication {{Patterns}} in {{Task}}-{{Oriented Groups}}},
  author = {Bavelas, Alex},
  year = {1950},
  month = nov,
  journal = {The Journal of the Acoustical Society of America},
  volume = {22},
  number = {6},
  pages = {725--730},
  publisher = {Acoustical Society of America},
  issn = {0001-4966},
  doi = {10.1121/1.1906679},
  urldate = {2023-03-28}
}

@article{barabasi2000scale,
  title={Scale-free characteristics of random networks: the topology of the world-wide web},
  author={Barab{\'a}si, Albert-L{\'a}szl{\'o} and Albert, R{\'e}ka and Jeong, Hawoong},
  journal={Physica A: Statistical Mechanics and its Applications},
  volume={281},
  number={1-4},
  pages={69--77},
  year={2000},
  publisher={Elsevier}
}

@article{bokanyiAnatomyPopulationscaleSocial2023,
  title = {The Anatomy of a Population-Scale Social Network},
  author = {Bok{\'a}nyi, Eszter and Heemskerk, Eelke M. and Takes, Frank W.},
  year = {2023},
  month = jun,
  journal = {Scientific Reports},
  volume = {13},
  number = {1},
  pages = {9209},
  publisher = {Nature Publishing Group},
  issn = {2045-2322},
  doi = {10.1038/s41598-023-36324-9},
}

@article{bokanyiUrbanHierarchySpatial2022a,
  title = {Urban Hierarchy and Spatial Diffusion over the Innovation Life Cycle},
  author = {Bok{\'a}nyi, Eszter and Nov{\'a}k, Martin and Jakobi, {\'A}kos and Lengyel, Bal{\'a}zs},
  year = {2022},
  month = may,
  journal = {Royal Society Open Science},
  volume = {9},
  number = {5},
  pages = {211038},
  publisher = {Royal Society},
  doi = {10.1098/rsos.211038},
  urldate = {2024-09-27},
  abstract = {Successful innovations achieve large geographical coverage by spreading across settlements and distances. For decades, spatial diffusion has been argued to take place along the urban hierarchy. Yet, the role of geographical distance was difficult to identify in hierarchical diffusion due to missing data on spreading events. In this paper, we exploit spatial patterns of individual invitations sent from registered users to new users over the entire life cycle of a social media platform. We demonstrate that hierarchical diffusion overlaps with diffusion to close distances and these factors co-evolve over the life cycle. Therefore, we disentangle them in a regression framework that estimates the yearly number of invitations sent between pairs of towns. We confirm that hierarchical diffusion prevails initially across large towns only but emerges in the full spectrum of settlements in the middle of the life cycle when adoption accelerates. Unlike in previous gravity estimations, we find that after an intensifying role of distance in the middle of the life cycle a surprisingly weak distance effect characterizes the last years of diffusion. Our results stress the dominance of urban hierarchy in spatial diffusion and inform future predictions of innovation adoption at local scales.},
  keywords = {diffusion,hierarchical diffusion,innovation,neighbourhood diffusion,social networks},
  file = {C:\Users\niekk\Zotero\storage\4H6SKFWP\Bokányi et al. - 2022 - Urban hierarchy and spatial diffusion over the inn.pdf}
}

@book{boydCultureEvolutionaryProcess1985,
  title = {Culture and the Evolutionary Process},
  author = {Boyd, Robert and Richerson, Peter J.},
  year = {1985},
  publisher = {University of Chicago Press},
  address = {Chicago, IL},
  isbn = {978-0226066827}
}

@article{canteloupWildPrimatesCopy2020,
  title = {Wild Primates Copy Higher-Ranked Individuals in a Social Transmission Experiment},
  author = {Canteloup, Charlotte and Hoppitt, William and {van de Waal}, Erica},
  year = {2020},
  month = jan,
  journal = {Nature Communications},
  volume = {11},
  number = {1},
  pages = {459},
  publisher = {Nature Publishing Group},
  issn = {2041-1723},
  doi = {10.1038/s41467-019-14209-8},
  urldate = {2024-09-10},
  abstract = {Little is known about how multiple social learning strategies interact and how organisms integrate both individual and social information. Here we combine, in a wild primate, an open diffusion experiment with a modeling approach: Network-Based Diffusion Analysis using a dynamic observation network. The vervet monkeys we study were not provided with a trained model; instead they had access to eight foraging boxes that could be opened in either of two ways. We report that individuals socially learn the techniques they observe in others. After having learnt one option, individuals are 31x more likely to subsequently asocially learn the other option than individuals na{\"i}ve to both options. We discover evidence of a rank transmission bias favoring learning from higher-ranked individuals, with no evidence for age, sex or kin bias. This fine-grained analysis highlights a rank transmission bias in a field experiment mimicking the diffusion of a behavioral innovation.},
  copyright = {2020 The Author(s)},
  langid = {english},
  keywords = {Cultural evolution,Social evolution},
  file = {C:\Users\niekk\Zotero\storage\JLHWYFMU\Canteloup et al. - 2020 - Wild primates copy higher-ranked individuals in a .pdf}
}

@article{cantorInterplaySocialNetworks2013,
  title = {The Interplay between Social Networks and Culture: Theoretically and among Whales and Dolphins},
  shorttitle = {The Interplay between Social Networks and Culture},
  author = {Cantor, Mauricio and Whitehead, Hal},
  year = {2013},
  month = may,
  journal = {Philosophical Transactions of the Royal Society B: Biological Sciences},
  volume = {368},
  number = {1618},
  pages = {20120340},
  issn = {0962-8436},
  doi = {10.1098/rstb.2012.0340},
  urldate = {2023-03-31},
  abstract = {Culture is increasingly being understood as a driver of mammalian phenotypes. Defined as group-specific behaviour transmitted by social learning, culture is shaped by social structure. However, culture can itself affect social structure if individuals preferentially interact with others whose behaviour is similar, or cultural symbols are used to mark groups. Using network formalism, this interplay can be depicted by the coevolution of nodes and edges together with the coevolution of network topology and transmission patterns. We review attempts to model the links between the spread, persistence and diversity of culture and the network topology of non-human societies. We illustrate these processes using cetaceans. The spread of socially learned begging behaviour within a population of bottlenose dolphins followed the topology of the social network, as did the evolution of the song of the humpback whale between breeding areas. In three bottlenose dolphin populations, individuals preferentially associated with animals using the same socially learned foraging behaviour. Homogeneous behaviour within the tight, nearly permanent social structures of the large matrilineal whales seems to result from transmission bias, with cultural symbols marking social structures. We recommend the integration of studies of culture and society in species for which social learning is an important determinant of behaviour.},
  pmcid = {PMC3638443},
  pmid = {23569288},
  file = {C:\Users\niekk\Zotero\storage\TCFDEN6R\Cantor and Whitehead - 2013 - The interplay between social networks and culture.pdf}
}

@article{centolaComplexContagionsWeakness2007,
  title = {Complex {{Contagions}} and the {{Weakness}} of {{Long Ties}}},
  author = {Centola, Damon and Macy, Michael},
  year = {2007},
  month = nov,
  journal = {American Journal of Sociology},
  volume = {113},
  number = {3},
  pages = {702--734},
  issn = {0002-9602, 1537-5390},
  doi = {10.1086/521848},
  urldate = {2024-09-11},
  abstract = {The strength of weak ties is that they tend to be long---they connect socially distant locations, allowing information to diffuse rapidly. The authors test whether this ``strength of weak ties'' generalizes from simple to complex contagions. Complex contagions require social affirmation from multiple sources. Examples include the spread of high-risk social movements, avant garde fashions, and unproven technologies. Results show that as adoption thresholds increase, long ties can impede diffusion. Complex contagions depend primarily on the width of the bridges across a network, not just their length. Wide bridges are a characteristic feature of many spatial networks, which may account in part for the widely observed tendency for social movements to diffuse spatially.},
  langid = {english},
  file = {C:\Users\niekk\Zotero\storage\UUYDM9YR\Centola and Macy - 2007 - Complex Contagions and the Weakness of Long Ties.pdf}
}

@article{centolaNetworkScienceCollective2022,
  title = {The Network Science of Collective Intelligence},
  author = {Centola, Damon},
  year = {2022},
  month = nov,
  journal = {Trends in Cognitive Sciences},
  volume = {26},
  number = {11},
  pages = {923--941},
  issn = {1364-6613},
  doi = {10.1016/j.tics.2022.08.009},
  urldate = {2023-02-06},
  abstract = {In the last few years, breakthroughs in computational and experimental techniques have produced several key discoveries in the science of networks and human collective intelligence. This review presents the latest scientific findings from two key fields of research: collective problem-solving and the wisdom of the crowd. I demonstrate the core theoretical tensions separating these research traditions and show how recent findings offer a new synthesis for understanding how network dynamics alter collective intelligence, both positively and negatively. I conclude by highlighting current theoretical problems at the forefront of research on networked collective intelligence, as well as vital public policy challenges that require new research efforts.},
  langid = {english},
  keywords = {collective intelligence,collective problem-solving,networks,wisdom of the crowd},
  file = {C:\Users\niekk\Zotero\storage\YW7G7WGD\S1364661322002054.html}
}

@article{centolaSpontaneousEmergenceConventions2015,
  title = {The {{Spontaneous Emergence}} of {{Conventions}}: {{An Experimental Study}} of {{Cultural Evolution}}},
  shorttitle = {The {{Spontaneous Emergence}} of {{Conventions}}},
  author = {Centola, Damon and Baronchelli, Andrea},
  year = {2015},
  month = feb,
  journal = {Proceedings of the National Academy of Sciences of the United States of America},
  volume = {112},
  number = {7},
  pages = {1989--1994},
  doi = {10.1073/pnas.1418838112},
  abstract = {Significance Social conventions shape every aspect of our lives, from how we greet each other to the languages we speak. Yet their origins have been a topic of theoretical speculation since the time of Aristotle. Most approaches assume that institutions are necessary to organize large populations, but the simplest explanation is that universally accepted conventions are the unintended consequence of individuals' efforts to coordinate locally with one another. Although this hypothesis is compelling, it lacks conclusive empirical support. Here, we present results from controlled experiments demonstrating that changes in network connectivity can cause global social conventions to spontaneously emerge from local interactions, even though people have no knowledge about the population, or that they are coordinating at a global scale.},
  file = {C:\Users\niekk\Zotero\storage\N2HNLFI5\Centola and Baronchelli - 2015 - The Spontaneous Emergence of Conventions An Exper.pdf}
}

@article{centolaSpreadBehaviorOnline2010,
  title = {The {{Spread}} of {{Behavior}} in an {{Online Social Network Experiment}}},
  author = {Centola, Damon},
  year = {2010},
  month = sep,
  journal = {Science},
  volume = {329},
  number = {5996},
  pages = {1194--1197},
  issn = {0036-8075, 1095-9203},
  doi = {10.1126/science.1185231},
  urldate = {2023-03-28},
  abstract = {Join the Club                            An important question for policy-makers is how to communicate information (for example, about public health interventions) and promote behavior change most effectively across a population. The structure of a social network can dramatically affect the diffusion of behavior through a population.               Centola               (p.               1194               ) examined whether the number of individuals choosing to register for a health forum could be influenced by an artificially constructed network of neighbors that were signed up for the forum. The behavior spread more readily on clustered networks than on random, poorly clustered ones. Certain types of behavior within human systems are thus more likely to spread if people are exposed to many other people who have already adopted the behavior (for example, in the circumstances where your friends know each other, as well as yourself).                        ,              An online experiment shows how network structure affects the spread of health behavior.           ,              How do social networks affect the spread of behavior? A popular hypothesis states that networks with many clustered ties and a high degree of separation will be less effective for behavioral diffusion than networks in which locally redundant ties are rewired to provide shortcuts across the social space. A competing hypothesis argues that when behaviors require social reinforcement, a network with more clustering may be more advantageous, even if the network as a whole has a larger diameter. I investigated the effects of network structure on diffusion by studying the spread of health behavior through artificially structured online communities. Individual adoption was much more likely when participants received social reinforcement from multiple neighbors in the social network. The behavior spread farther and faster across clustered-lattice networks than across corresponding random networks.},
  langid = {english},
  file = {C:\Users\niekk\Zotero\storage\LRKCHAN5\Centola - 2010 - The Spread of Behavior in an Online Social Network.pdf}
}

@article{chimentoContributionMovementSocial2024,
  title = {The Contribution of Movement to Social Network Structure and Spreading Dynamics under Simple and Complex Transmission},
  author = {Chimento, Michael and Farine, Damien R.},
  year = {2024},
  month = oct,
  journal = {Philosophical Transactions of the Royal Society B: Biological Sciences},
  volume = {379},
  number = {1912},
  pages = {20220524},
  issn = {0962-8436, 1471-2970},
  doi = {10.1098/rstb.2022.0524},
  urldate = {2024-09-11},
  abstract = {The structure of social networks fundamentally influences spreading dynamics. In general, the more contact between individuals, the more opportunity there is for the transmission of information or disease to take place. Yet, contact between individuals, and any resulting transmission events, are determined by a combination of spatial (where individuals choose to move) and social rules (who they choose to interact with or learn from). Here, we examine the effect of the social--spatial interface on spreading dynamics using a simulation model. We quantify the relative effects of different movement rules (localized, semi-localized, nomadic and resource-based movement) and social transmission rules (simple transmission, anti-conformity, proportional, conformity and threshold rules) to both the structure of social networks and spread of a novel behaviour. Localized movement created weakly connected sparse networks, nomadic movement created weakly connected dense networks, and resource-based movement generated strongly connected modular networks. The resulting rate of spreading varied with different combinations of movement and transmission rules, but---importantly---the relative rankings of transmission rules changed when running simulations on static versus dynamic representations of networks. Our results emphasize that individual-level social and spatial behaviours influence emergent network structure, and are of particular consequence for the spread of information under complex transmission rules.             This article is part of the theme issue `The spatial--social interface: a theoretical and empirical integration'.},
  langid = {english},
  file = {C:\Users\niekk\Zotero\storage\KKD6VH7X\Chimento and Farine - 2024 - The contribution of movement to social network str.pdf}
}

@article{conteStrategiesSocialNetwork,
  title = {Strategies in Social Network Formation},
  author = {Conte, Anna and Di Cagno, Daniela and Sciubba, Emanuela},
  journal = {Theory and Decision},
  volume = {67},
  number = {2},
  pages = {161--193},
  year = {2009},
  abstract = {We run a computerised experiment of network formation where all connections are beneficial and only direct links are costly. Players simultaneously submit link proposals; a connection is made only when both players involved agree. We use both simulated and experimentally generated data to test the determinants of individual behaviour in network formation. We find that approximately 40\% of the network formation strategies adopted by the experimental subjects can be accounted for as best responses. We test whether subjects follow alternative patterns of behaviour and in particular if they: propose links to those from whom they have received link proposals in the previous round; propose links to those who have the largest number of direct connections. We find that together with best response behaviour, these strategies explain approximately 75\% of the observed choices. We estimate individual propensities to adopt each of these strategies, controlling for group effects. Finally, we estimate a mixture model to highlight the proportion of each type of decision maker in the population.},
  langid = {english},
  file = {C:/Users/niekk/Zotero/storage/IE932S4S/Conte et al. - Strategies in Social Network Formation.pdf}
}


@incollection{cowgillUsingPredictionMarkets2009,
  title = {Using {{Prediction Markets}} to {{Track Information Flows}}: {{Evidence}} from {{Google}}},
  shorttitle = {Using {{Prediction Markets}} to {{Track Information Flows}}},
  booktitle = {Auctions, {{Market Mechanisms}} and {{Their Applications}}},
  author = {Cowgill, Bo and Wolfers, Justin and Zitzewitz, Eric},
  editor = {Das, Sanmay and Ostrovsky, Michael and Pennock, David and Szymanksi, Boleslaw},
  year = {2009},
  volume = {14},
  pages = {3--3},
  publisher = {Springer Berlin Heidelberg},
  address = {Berlin, Heidelberg},
  doi = {10.1007/978-3-642-03821-1_2},
  urldate = {2023-03-28},
  abstract = {In the last three years, Google has conducted the largest corporate experiment with prediction markets we are aware of. In this paper, we illustrate how markets can be used to study how an organization processes information. We document a number of biases in Google's markets, most notably an optimistic bias. Newly hired employees are on the optimistic side of these markets, and optimistic biases are significantly more pronounced on days when Google stock is appreciating. We find correlated trading among employees who sit within a few feet of one another and employees with social or work relationships. The results are interesting in light of recent research on the role of optimism in entrepreneurial firms, as well as recent work on the importance of geographic and social proximity in explaining information flows in firms and markets.},
  isbn = {978-3-642-03820-4 978-3-642-03821-1},
  langid = {english},
  file = {C:\Users\niekk\Zotero\storage\B6RZ76D4\Cowgill et al. - 2009 - Using Prediction Markets to Track Information Flow.pdf}
}

@article{deffnerEffectivePopulationSize2021,
  title = {Effective Population Size for Culturally Evolving Traits},
  author = {Deffner, Dominik and Kandler, Anne and Fogarty, Laurel},
  year = {2021},
  month = sep,
  journal = {bioRxiv},
  abstract = {This article presents research on the concept of effective population size for cultural traits, exploring how it impacts the evolution and transmission of these traits in populations. The authors investigate the implications for both innovation and cultural inheritance in small versus large populations, providing a mathematical framework and empirical discussion.},
  file = {C:/Users/niekk/Zotero/storage/8HHSIV6B/Deffner et al. - 2021 - Effective population size for culturally evolving.pdf}
}

@article{derexDivideConquerIntermediate2018,
  title = {Divide and Conquer: Intermediate Levels of Population Fragmentation Maximize Cultural Accumulation},
  shorttitle = {Divide and Conquer},
  author = {Derex, Maxime and Perreault, Charles and Boyd, Robert},
  year = {2018},
  month = feb,
  journal = {Philosophical Transactions of the Royal Society B: Biological Sciences},
  volume = {373},
  number = {1743},
  pages = {20170062},
  publisher = {Royal Society},
  doi = {10.1098/rstb.2017.0062},
  urldate = {2023-03-28},
  abstract = {Identifying the determinants of cumulative cultural evolution is a key issue in the interdisciplinary field of cultural evolution. A widely held view is that large and well-connected social networks facilitate cumulative cultural evolution because they promote the spread of useful cultural traits and prevent the loss of cultural knowledge through factors such as drift. This view stems from models that focus on the transmission of cultural information, without considering how new cultural traits actually arise. In this paper, we review the literature from various fields that suggest that, under some circumstances, increased connectedness can decrease cultural diversity and reduce innovation rates. Incorporating this idea into an agent-based model, we explore the effect of population fragmentation on cumulative culture and show that, for a given population size, there exists an intermediate level of population fragmentation that maximizes the rate of cumulative cultural evolution. This result is explained by the fact that fully connected, non-fragmented populations are able to maintain complex cultural traits but produce insufficient variation and so lack the cultural diversity required to produce highly complex cultural traits. Conversely, highly fragmented populations produce a variety of cultural traits but cannot maintain complex ones. In populations with intermediate levels of fragmentation, cultural loss and cultural diversity are balanced in a way that maximizes cultural complexity. Our results suggest that population structure needs to be taken into account when investigating the relationship between demography and cumulative culture. This article is part of the theme issue `Bridging cultural gaps: interdisciplinary studies in human cultural evolution'.},
  keywords = {cultural convergence,cultural homogenization,innovation,population structure,social learning,technological trajectory},
  file = {C:\Users\niekk\Zotero\storage\6DTHD2BW\Derex et al. - 2018 - Divide and conquer intermediate levels of populat.pdf}
}

@article{derexPartialConnectivityIncreases2016,
  title = {Partial Connectivity Increases Cultural Accumulation within Groups},
  author = {Derex, Maxime and Boyd, Robert},
  year = {2016},
  month = mar,
  journal = {Proceedings of the National Academy of Sciences},
  volume = {113},
  number = {11},
  pages = {2982--2987},
  publisher = {Proceedings of the National Academy of Sciences},
  doi = {10.1073/pnas.1518798113},
  urldate = {2023-02-06},
  abstract = {Complex technologies used in most human societies are beyond the inventive capacities of individuals. Instead, they result from a cumulative process in which innovations are gradually added to existing cultural traits across many generations. Recent work suggests that a population's ability to develop complex technologies is positively affected by its size and connectedness. Here, we present a simple computer-based experiment that compares the accumulation of innovations by fully and partially connected groups of the same size in a complex fitness landscape. We find that the propensity to learn from successful individuals drastically reduces cultural diversity within fully connected groups. In comparison, partially connected groups produce more diverse solutions, and this diversity allows them to develop complex solutions that are never produced in fully connected groups. These results suggest that explanations of ancestral patterns of cultural complexity may need to consider levels of population fragmentation and interaction patterns between partially isolated groups.},
  file = {C:\Users\niekk\Zotero\storage\TVCAI7AA\Derex and Boyd - 2016 - Partial connectivity increases cultural accumulati.pdf}
}

@article{erdos1959random,
  title={On random graphs},
  author={Erd{\H{o}}s, Paul and R{\'e}nyi, Alfr{\'e}d},
  journal={Publicationes Mathematicae Debrecen},
  volume={6},
  pages={290--297},
  year={1959}
}

@article{gemarParentalStatusConnection2024,
  title = {Parental {{Status Connection}} and {{Social Network Variety}} in {{Adulthood}}},
  author = {Gemar, Adam},
  year = {2024},
  month = feb,
  journal = {Societies},
  volume = {14},
  pages = {26},
  doi = {10.3390/soc14020026},
  abstract = {This study enriches the literature on social networks and social capital by investigating how parental status potentially impacts social network diversity in adulthood. Using the 2018 iteration of the General Social Survey (GSS, n = 2348), a high quality nationally representative survey of the United States, we utilize latent class and regression analyses, finding that parental status, especially medium and cross-status occupational connections contribute to social capital in the form of network diversity. Yet, personal socio-economic factors, notably income and race, largely offset parental effects. This underscores the complexity of network composition, emphasizing the influential role of individual resources, attributes, and mobility in shaping social networks and forming bridging social capital.},
  file = {C:\Users\niekk\Zotero\storage\23WA7SIU\Gemar - 2024 - Parental Status Connection and Social Network Vari.pdf}
}

@article{gonzalezUnderstandingIndividualHuman2008,
  title = {Understanding {{Individual Human Mobility Patterns}}},
  author = {Gonzalez, Marta C. and Hidalgo, Cesar and Barabasi, Albert-Laszlo},
  year = {2008},
  month = jul,
  journal = {Nature},
  volume = {453},
  pages = {779--82},
  doi = {10.1038/nature06958},
  abstract = {Despite their importance for urban planning, traffic forecasting and the spread of biological and mobile viruses, our understanding of the basic laws governing human motion remains limited owing to the lack of tools to monitor the time-resolved location of individuals. Here we study the trajectory of 100,000 anonymized mobile phone users whose position is tracked for a six-month period. We find that, in contrast with the random trajectories predicted by the prevailing L{\'e}vy flight and random walk models, human trajectories show a high degree of temporal and spatial regularity, each individual being characterized by a time-independent characteristic travel distance and a significant probability to return to a few highly frequented locations. After correcting for differences in travel distances and the inherent anisotropy of each trajectory, the individual travel patterns collapse into a single spatial probability distribution, indicating that, despite the diversity of their travel history, humans follow simple reproducible patterns. This inherent similarity in travel patterns could impact all phenomena driven by human mobility, from epidemic prevention to emergency response, urban planning and agent-based modelling.},
  file = {C:\Users\niekk\Zotero\storage\96GUV7NT\Gonzalez et al. - 2008 - Understanding Individual Human Mobility Patterns.pdf}
}

@article{henrichDemographyCulturalEvolution2004,
  title = {Demography and {{Cultural Evolution}}: {{How Adaptive Cultural Processes Can Produce Maladaptive Losses}}---{{The Tasmanian Case}}},
  shorttitle = {Demography and {{Cultural Evolution}}},
  author = {Henrich, Joseph},
  year = {2004},
  month = apr,
  journal = {American Antiquity},
  volume = {69},
  number = {2},
  pages = {197--214},
  issn = {0002-7316, 2325-5064},
  doi = {10.2307/4128416},
  urldate = {2024-09-11},
  abstract = {A combination of archeological and ethnohistorical evidence indicates that, over an approximately 8,000-year period, from the beginning of the Holocene until European explorers began arriving in the eighteenth century, the societies of Tasmania lost a series of valuable skills and technologies. These likely included bone tools, cold-weather clothing, hafted tools, nets, fishing spears, barbed spears, spear-throwers, and boomerangs. To address this puzzle, and the more general question of how human cognition and social interaction can generate both adaptive cultural evolution and maladaptive losses of culturally acquired skills, this paper constructs a formal model of cultural evolution rooted in the cognitive details of human social learning and inference. The analytical results specify the conditions for differing rates of adaptive cultural evolution, and reveal regimes that will produce maladaptive losses of particular kinds of skills and related technologies. More specifically, the results suggest that the relatively sudden reduction in the effective population size (the size of the interacting pool of social learners) that occurred with the rising ocean levels at the end of the last glacial epoch, which cut Tasmania off from the rest of Australia for the ensuing ten millennia, could have initiated a cultural evolutionary process that (1) kept stable or even improved relatively simple technological skills, and (2) produced an increasing deterioration of more complex skills leading to the complete disappearance of some technologies and practices. This pattern is consistent with the empirical record in Tasmania. Beyond this case, I speculate on the applicability of the model to understanding the variability in rates of adaptive cultural evolution.           ,              Resumen             La evidencia arqueol{\'o}gica y etnohist{\'o}rica indica que, a lo largo de aproximadamente 8,000 a{\~n}os, desde el principio del Holoceno hasta la llegada de exploradores europeos en el sigh XVIII, las sociedades de Tasmania perdieron gran parte de su cultura tecnol{\'o}gica. Las herramientas que desaparecieron probablemente incluyen el hueso, ropa resistente al fr{\'i}o, los instrumentos enmangados, arpones, lanzas de p{\'u}as, los lanza-lanzadores y los bumerangs. {\textquestiondown}C{\'o}mo es posible que se perdiera todo esto? Para resolver este misterio, y tambi{\'e}n esclarecer deforma m{\'a}s general c{\'o}mo el conocimiento humano y la interacci{\'o}n social pueden generar adaptaciones y tambi{\'e}n la p{\'e}rdida de las mismas, e inclusive malas adaptaciones, en este art{\'i}culo se construye un modelo formal de la evoluci{\'o}n cultural que se basa en detalles cognoscitivos del aprendizaje y la inferencia humanos en el {\'a}mbito social. Los resultados anal{\'i}ticos especifican los reg{\'i}menes de condiciones bajo los cuales la evoluci{\'o}n cultural genera adaptaciones, y tambi{\'e}n los reg{\'i}menes contrastantes bajo los cuales seproducen p{\'e}rdidas que representan malas adaptaciones tanto de habilidades como de las tecnolog{\'i}as vinculadas con ellas. M{\'a}s espec{\'i}ficamente, los resultados sugieren que la reducci{\'o}n relativamente repentina en el tama{\~n}o eficaz de la poblaci{\'o}n (el tama{\~n}o del grupo de aprendices sociales), es la causa m{\'a}s importante de estas p{\'e}rdidas culturales. El motor ecol{\'o}gico de esta reducci{\'o}n fue el alza del nivel del mar en la {\'e}poca final de la glaciaci{\'o}n pasada, que tuvo como efecto separar a Tasmania del resto de Australia durante los {\'u}ltimos diez milenios. La consecuencia fue un deterioro de las habilidades m{\'a}s complejas con las cuales contaba esta poblaci{\'o}n. El expediente empir{\'i}co de la arqueolog{\'i}a en Tasmania confirma este patr{\'o}n. M{\'a}s all{\'a} de este caso particular, se presentan especulaciones acerca de la aplicabilidad de este modelo para entender la variabilidad en los {\'i}ndices de la evoluci{\'o}n cultural adaptativa en el marco tecnol{\'o}gico.},
  copyright = {https://www.cambridge.org/core/terms},
  langid = {english},
  file = {C:\Users\niekk\Zotero\storage\6NYD2UQM\Henrich - 2004 - Demography and Cultural Evolution How Adaptive Cu.pdf}
}

@article{humphriesNetworkSmallWorldNessQuantitative2008,
  title = {Network `{{Small-World-Ness}}': {{A Quantitative Method}} for {{Determining Canonical Network Equivalence}}},
  shorttitle = {Network `{{Small-World-Ness}}'},
  author = {Humphries, Mark D. and Gurney, Kevin},
  editor = {Sporns, Olaf},
  year = {2008},
  month = apr,
  journal = {PLoS ONE},
  volume = {3},
  number = {4},
  pages = {e0002051},
  issn = {1932-6203},
  doi = {10.1371/journal.pone.0002051},
  urldate = {2023-05-08},
  abstract = {Background: Many technological, biological, social, and information networks fall into the broad class of `small-world' networks: they have tightly interconnected clusters of nodes, and a shortest mean path length that is similar to a matched random graph (same number of nodes and edges). This semi-quantitative definition leads to a categorical distinction (`small/not-small') rather than a quantitative, continuous grading of networks, and can lead to uncertainty about a network's small-world status. Moreover, systems described by small-world networks are often studied using an equivalent canonical network model -- the Watts-Strogatz (WS) model. However, the process of establishing an equivalent WS model is imprecise and there is a pressing need to discover ways in which this equivalence may be quantified. Methodology/Principal Findings: We defined a precise measure of `small-world-ness' S based on the trade off between high local clustering and short path length. A network is now deemed a `small-world' if S.1 - an assertion which may be tested statistically. We then examined the behavior of S on a large data-set of real-world systems. We found that all these systems were linked by a linear relationship between their S values and the network size n. Moreover, we show a method for assigning a unique Watts-Strogatz (WS) model to any real-world network, and show analytically that the WS models associated with our sample of networks also show linearity between S and n. Linearity between S and n is not, however, inevitable, and neither is S maximal for an arbitrary network of given size. Linearity may, however, be explained by a common limiting growth process. Conclusions/Significance: We have shown how the notion of a small-world network may be quantified. Several key properties of the metric are described and the use of WS canonical models is placed on a more secure footing.},
  langid = {english},
  file = {C:\Users\niekk\Zotero\storage\V4QI9A8C\Humphries and Gurney - 2008 - Network ‘Small-World-Ness’ A Quantitative Method .pdf}
}

@article{ilanyRankdependentSocialInheritance2021,
  title = {Rank-Dependent Social Inheritance Determines Social Network Structure in Spotted Hyenas},
  author = {Ilany, Amiyaal and Holekamp, Kay E. and Ak{\c c}ay, Erol},
  year = {2021},
  month = jul,
  journal = {Science (New York, N.Y.)},
  volume = {373},
  number = {6552},
  pages = {348--352},
  issn = {1095-9203},
  doi = {10.1126/science.abc1966},
  abstract = {The structure of animal social networks influences survival and reproductive success, as well as pathogen and information transmission. However, the general mechanisms determining social structure remain unclear. Using data from 73,767 social interactions among wild spotted hyenas collected over 27 years, we show that the process of social inheritance determines how offspring relationships are formed and maintained. Relationships between offspring and other hyenas bear resemblance to those of their mothers for as long as 6 years, and the degree of similarity increases with maternal social rank. Mother-offspring relationship strength affects social inheritance and is positively correlated with offspring longevity. These results support the hypothesis that social inheritance of relationships can structure animal social networks and be subject to adaptive tradeoffs.},
  langid = {english},
  pmid = {34437155},
  keywords = {Animals,Behavior Animal,Female,Hierarchy Social,Hyaenidae,Longevity,Male,Mothers,Social Behavior,Social Interaction,Social Networking},
  file = {C:\Users\niekk\Zotero\storage\EAEJL52B\Ilany et al. - 2021 - Rank-dependent social inheritance determines socia.pdf}
}

@article{kendalChimpanzeesCopyDominant2015,
  title = {Chimpanzees Copy Dominant and Knowledgeable Individuals: Implications for Cultural Diversity},
  shorttitle = {Chimpanzees Copy Dominant and Knowledgeable Individuals},
  author = {Kendal, Rachel and Hopper, Lydia M. and Whiten, Andrew and Brosnan, Sarah F. and Lambeth, Susan P. and Schapiro, Steven J. and Hoppitt, Will},
  year = {2015},
  month = jan,
  journal = {Evolution and Human Behavior},
  volume = {36},
  number = {1},
  pages = {65--72},
  issn = {10905138},
  doi = {10.1016/j.evolhumbehav.2014.09.002},
  urldate = {2024-09-10},
  abstract = {Semantic Scholar extracted view of "Chimpanzees copy dominant and knowledgeable individuals: implications for cultural diversity." by R. Kendal et al.},
  langid = {english},
  file = {C:\Users\niekk\Zotero\storage\WA2MF3NJ\Kendal et al. - 2015 - Chimpanzees copy dominant and knowledgeable indivi.pdf}
}

@article{kendalSocialLearningStrategies2018,
  title = {Social {{Learning Strategies}}: {{Bridge-Building}} between {{Fields}}},
  shorttitle = {Social {{Learning Strategies}}},
  author = {Kendal, Rachel L. and Boogert, Neeltje J. and Rendell, Luke and Laland, Kevin N. and Webster, Mike and Jones, Patricia L.},
  year = {2018},
  month = jul,
  journal = {Trends in Cognitive Sciences},
  volume = {22},
  number = {7},
  pages = {651--665},
  publisher = {Elsevier},
  issn = {1364-6613, 1879-307X},
  doi = {10.1016/j.tics.2018.04.003},
  urldate = {2024-09-10},
  langid = {english},
  pmid = {29759889},
  keywords = {asocial information,associative learning theory,behavioural gambit,cumulative culture,metacognition,social information},
  file = {C:\Users\niekk\Zotero\storage\6PWAY92E\Kendal et al. - 2018 - Social Learning Strategies Bridge-Building betwee.pdf}
}

@incollection{kotaInsectCommunication2022,
  title = {Insect Communication},
  author = {Kota, Mounica and Olzer, Rachel},
  booktitle = {Encyclopedia of Animal Cognition and Behavior},
  editor = {Vonk, Jennifer and Shackelford, Todd K.},
  year = {2022},
  month = may,
  pages = {3465--3471},
  isbn = {978-3-319-55064-0}
}

@article{lalandSocialLearningStrategies2004,
  title = {Social Learning Strategies},
  author = {Laland, Kevin N.},
  year = {2004},
  month = feb,
  journal = {Learning \& Behavior},
  volume = {32},
  number = {1},
  pages = {4--14},
  issn = {1543-4508},
  doi = {10.3758/BF03196002},
  urldate = {2024-09-10},
  abstract = {In most studies of social learning in animals, no attempt has been made to examine the nature of the strategy adopted by animals when they copy others. Researchers have expended considerable effort in exploring the psychological processes that underlie social learning and amassed extensive data banks recording purported social learning in the field, but the contexts under which animals copy others remain unexplored. Yet, theoretical models used to investigate the adaptive advantages of social learning lead to the conclusion that social learning cannot be indiscriminate and that individuals should adopt strategies that dictate the circumstances under which they copy others and from whom they learn. In this article, I discuss a number of possible strategies that are predicted by theoretical analyses, includingcopy when uncertain,copy the majority, andcopy if better, and consider the empirical evidence in support of each, drawing from both the animal and human social learning literature. Reliance on social learning strategies may be organized hierarchically, their being employed by animals when unlearned and asocially learned strategies prove ineffective but before animals take recourse in innovation.},
  langid = {english},
  keywords = {Animal Behaviour,Artificial Intelligence,Mate Choice,Niche Construction,Social Learning,Zebra Finch},
  file = {C:\Users\niekk\Zotero\storage\AN9ZWEWV\Laland - 2004 - Social learning strategies.pdf}
}

@article{langbauerElephantCommunication2000,
  title = {Elephant Communication},
  author = {Langbauer, W.R.},
  year = {2000},
  journal = {Zoo Biology},
  volume = {19},
  number = {5},
  pages = {425--445},
  issn = {0733-3188, 1098-2361},
  doi = {10.1002/1098-2361(2000)19:5<425::AID-ZOO11>3.0.CO;2-A},
  urldate = {2023-08-01},
  langid = {english}
}

@article{lazerNetworkStructureExploration2007,
  title = {The {{Network Structure}} of {{Exploration}} and {{Exploitation}}},
  author = {Lazer, David and Friedman, Allan},
  year = {2007},
  month = dec,
  journal = {Administrative Science Quarterly},
  volume = {52},
  number = {4},
  pages = {667--694},
  issn = {0001-8392, 1930-3815},
  doi = {10.2189/asqu.52.4.667},
  urldate = {2024-09-10},
  abstract = {Whether as team members brainstorming or cultures experimenting with new technologies, problem solvers communicate and share ideas. This paper examines how the structure of communication networks among actors can affect system-level performance. We present an agent-based computer simulation model of information sharing in which the less successful emulate the more successful. Results suggest that when agents are dealing with a complex problem, the more efficient the network at disseminating information, the better the short-run but the lower the long-run performance of the system. The dynamic underlying this result is that an inefficient network maintains diversity in the system and is thus better for exploration than an efficient network, supporting a more thorough search for solutions in the long run. For intermediate time frames, there is an inverted-U relationship between connectedness and performance, in which both poorly and well-connected systems perform badly, and moderately connected systems perform best. This curvilinear relationship between connectivity and group performance can be seen in several diverse instances of organizational and social behavior.},
  copyright = {https://journals.sagepub.com/page/policies/text-and-data-mining-license},
  langid = {english},
  file = {C:\Users\niekk\Zotero\storage\VU44I5JF\Lazer and Friedman - 2007 - The Network Structure of Exploration and Exploitat.pdf}
}

@book{acerbiMesoudiSmollaIndividualBasedModels2022,
  author = {Acerbi, Alberto and Mesoudi, Alex and Smolla, Marco},
  title = {Individual-Based Models of Cultural Evolution: A Step-by-Step Guide Using R},
  publisher = {Routledge},
  year = {2022},
  address = {London},
  url={https://acerbialberto.com/IBM-cultevo/}
}


@article{miglianoHuntergathererMultilevelSociality2020a,
  title = {Hunter-Gatherer Multilevel Sociality Accelerates Cumulative Cultural Evolution},
  author = {Migliano, Andrea B. and Battiston, Federico and Viguier, Sylvain and Page, Abigail E. and Dyble, Mark and Schlaepfer, Rodolph and Smith, Daniel and Astete, Leonora and Ngales, Marilyn and {Gomez-Gardenes}, Jesus and Latora, Vito and Vinicius, Lucio},
  year = {2020},
  month = feb,
  journal = {Science Advances},
  volume = {6},
  number = {9},
  pages = {eaax5913},
  issn = {2375-2548},
  doi = {10.1126/sciadv.aax5913},
  urldate = {2024-09-11},
  abstract = {Hunter-gatherers from different bands form fluid social networks that facilitate cultural innovation through recombination of cultural traditions.           ,                             Although multilevel sociality is a universal feature of human social organization, its functional relevance remains unclear. Here, we investigated the effect of multilevel sociality on cumulative cultural evolution by using wireless sensing technology to map inter- and intraband social networks among Agta hunter-gatherers. By simulating the accumulation of cultural innovations over the real Agta multicamp networks, we demonstrate that multilevel sociality accelerates cultural differentiation and cumulative cultural evolution. Our results suggest that hunter-gatherer social structures [based on (i) clustering of families within camps and camps within regions, (ii) cultural transmission within kinship networks, and (iii) high intercamp mobility] may have allowed past and present hunter-gatherers to maintain cumulative cultural adaptation despite low population density, a feature that may have been critical in facilitating the global expansion of               Homo sapiens               .},
  langid = {english},
  file = {C:\Users\niekk\Zotero\storage\AUC44SC9\Migliano et al. - 2020 - Hunter-gatherer multilevel sociality accelerates c.pdf}
}

@article{momennejadCollectiveMindsSocial2021,
  title = {Collective Minds: Social Network Topology Shapes Collective Cognition},
  shorttitle = {Collective Minds},
  author = {Momennejad, Ida},
  year = {2021},
  month = dec,
  journal = {Philosophical Transactions of the Royal Society B: Biological Sciences},
  volume = {377},
  number = {1843},
  pages = {20200315},
  publisher = {Royal Society},
  doi = {10.1098/rstb.2020.0315},
  urldate = {2023-03-28},
  abstract = {Human cognition is not solitary, it is shaped by collective learning and memory. Unlike swarms or herds, human social networks have diverse topologies, serving diverse modes of collective cognition and behaviour. Here, we review research that combines network structure with psychological and neural experiments and modelling to understand how the topology of social networks shapes collective cognition. First, we review graph-theoretical approaches to behavioural experiments on collective memory, belief propagation and problem solving. These results show that different topologies of communication networks synchronize or integrate knowledge differently, serving diverse collective goals. Second, we discuss neuroimaging studies showing that human brains encode the topology of one's larger social network and show similar neural patterns to neural patterns of our friends and community ties (e.g. when watching movies). Third, we discuss cognitive similarities between learning social and non-social topologies, e.g. in spatial and associative learning, as well as common brain regions involved in processing social and non-social topologies. Finally, we discuss recent machine learning approaches to collective communication and cooperation in multi-agent artificial networks. Combining network science with cognitive, neural and computational approaches empowers investigating how social structures shape collective cognition, which can in turn help design goal-directed social network topologies. This article is part of a discussion meeting issue `The emergence of collective knowledge and cumulative culture in animals, humans and machines'.},
  keywords = {cognitive neuroscience,collective cognition,collective memory,human memory,network topology,social networks},
  file = {C:\Users\niekk\Zotero\storage\SCPFKPGC\Momennejad - 2021 - Collective minds social network topology shapes c.pdf}
}

@article{moserInnovationfacilitatingNetworksCreate,
  title = {Innovation-Facilitating Networks Create Inequality},
  author = {Moser, Cody and Smaldino, Paul E},
  journal = {Proceedings of the Royal Society B: Biological Sciences},
  year = {2023},
  volume = {290},
  number = {2003},
  pages = {20230672},
  doi = {10.1098/rspb.2023.0672},
  langid = {english},
  file = {C:/Users/niekk/Zotero/storage/ZXV4RN3E/Moser and Smaldino - Innovation-facilitating networks create inequality.pdf}
}

@article{mulderIntergenerationalWealthTransmission2009,
  title = {Intergenerational {{Wealth Transmission}} and the {{Dynamics}} of {{Inequality}} in {{Small-Scale Societies}}},
  author = {Mulder, Monique Borgerhoff and Bowles, Samuel and Hertz, Tom and Bell, Adrian and Beise, Jan and Clark, Greg and Fazzio, Ila and Gurven, Michael and Hill, Kim and Hooper, Paul L. and Irons, William and Kaplan, Hillard and Leonetti, Donna and Low, Bobbi and Marlowe, Frank and McElreath, Richard and Naidu, Suresh and Nolin, David and Piraino, Patrizio and Quinlan, Rob and Schniter, Eric and Sear, Rebecca and Shenk, Mary and Smith, Eric Alden and Von Rueden, Christopher and Wiessner, Polly},
  year = {2009},
  month = oct,
  journal = {Science},
  volume = {326},
  number = {5953},
  pages = {682--688},
  issn = {0036-8075, 1095-9203},
  doi = {10.1126/science.1178336},
  urldate = {2024-09-11},
  abstract = {Origins of Egalitarianism                            Wealthy contemporary societies exhibit varying extents of economic inequality, with the Nordic countries being relatively egalitarian, whereas there is a much larger gap between top and bottom in the United States.                                Borgerhoff Mulder                 et al.                              (p.               682               ; see the Perspective by                                Acemoglu and Robinson                              ) build a bare-bones model describing the intergenerational transmission of three different types of wealth---based on social networks, land and livestock, and physical and cognitive capacity---in four types of small-scale societies in which livelihoods depended primarily on hunting, herding, farming, or horticulture. Parameter estimates from a large-scale analysis of historical and ethnographic data were added to the model to reveal that the four types of societies display distinctive patterns of wealth transmission and that these patterns are associated with different extents of inequality.                        ,              Some types of wealth are strongly inherited and, hence, contribute to long-term economic inequality.           ,              Small-scale human societies range from foraging bands with a strong egalitarian ethos to more economically stratified agrarian and pastoral societies. We explain this variation in inequality using a dynamic model in which a population's long-run steady-state level of inequality depends on the extent to which its most important forms of wealth are transmitted within families across generations. We estimate the degree of intergenerational transmission of three different types of wealth (material, embodied, and relational), as well as the extent of wealth inequality in 21 historical and contemporary populations. We show that intergenerational transmission of wealth and wealth inequality are substantial among pastoral and small-scale agricultural societies (on a par with or even exceeding the most unequal modern industrial economies) but are limited among horticultural and foraging peoples (equivalent to the most egalitarian of modern industrial populations). Differences in the technology by which a people derive their livelihood and in the institutions and norms making up the economic system jointly contribute to this pattern.},
  langid = {english},
  file = {C:\Users\niekk\Zotero\storage\QA9W822E\Mulder et al. - 2009 - Intergenerational Wealth Transmission and the Dyna.pdf}
}

@article{nakayamaSocialInformationSpontaneous2019,
  title = {Social Information and Spontaneous Emergence of Leaders in Human Groups},
  author = {Nakayama, Shinnosuke and Krasner, Elizabeth and Zino, Lorenzo and Porfiri, Maurizio},
  year = {2019},
  month = feb,
  journal = {Journal of the Royal Society Interface},
  volume = {16},
  number = {151},
  issn = {1742-5662},
  doi = {10.1098/rsif.2018.0938},
  urldate = {2023-03-28},
  abstract = {Understanding the dynamics of social networks is the objective of interdisciplinary research ranging from animal collective behaviour to epidemiology, political science and marketing. Social influence is key to comprehending emergent group behaviour, but we know little about how inter-individual relationships emerge in the first place. We conducted an experiment where participants repeatedly performed a cognitive test in a small group. In each round, they were allowed to change their answers upon seeing the current answers of other members and their past performance in selecting correct answers. Rather than following a simple majority rule, participants granularly processed the performance of others in deciding how to change their answers. Toward a network model of the experiment, we associated a directed link of a time-varying network with every change in a participant's answer that mirrored the answer of another group member. The rate of growth of the network was not constant in time, whereby links were found to emerge faster as time progressed. Further, repeated interactions reinforced relationships between individuals' performance and their network centrality. Our results provide empirical evidence that inter-individual relationships spontaneously emerge in an adaptive way, where good performers rise as group leaders over time.},
  keywords = {Collective behaviour,Dynamic networks,Leadership,Network evolution,Opinion formation},
  file = {C:\Users\niekk\Zotero\storage\FIUXUFJ8\Nakayama et al. - 2019 - Social information and spontaneous emergence of le.pdf}
}

@article{newman2003structure,
  title={The structure and function of complex networks},
  author={Newman, Mark E. J.},
  journal={SIAM Review},
  volume={45},
  number={2},
  pages={167--256},
  year={2003},
  doi={10.1137/S003614450342480}
}

@article{onnelaStructureTieStrengths2007,
  title = {Structure and {{Tie Strengths}} in {{Mobile Communication Networks}}},
  author = {Onnela, Jukka-Pekka and Saram{\"a}ki, Jari and Hyv{\"o}nen, J and Szab{\'o}, G and Lazer, David and Kaski, Kimmo and Kert{\'e}sz, J{\'a}nos and Barab{\'a}si, A.-L},
  year = {2007},
  month = jun,
  journal = {Proceedings of the National Academy of Sciences of the United States of America},
  volume = {104},
  pages = {7332--6},
  doi = {10.1073/pnas.0610245104},
}

@article{pikettyCapitalTwentyFirstCentury2015,
  title = {About {{{\emph{Capital}}}}{\emph{ in the }}{{{\emph{Twenty-First Century}}}}},
  author = {Piketty, Thomas},
  year = {2015},
  month = may,
  journal = {American Economic Review},
  volume = {105},
  number = {5},
  pages = {48--53},
  issn = {0002-8282},
  doi = {10.1257/aer.p20151060},
  urldate = {2024-09-11},
  abstract = {In this article, I present three key facts about income and wealth inequality in the long run emerging from my book Capital in the Twenty-First Century and seek to sharpen and refocus the discussion about those trends. In particular, I clarify the role played by r {$>$} g in my analysis of wealth inequality. I also discuss some of the implications for optimal taxation, and the relation between capital-income ratios and capital shares.},
  langid = {english},
  file = {C:\Users\niekk\Zotero\storage\PGH3UEYV\Piketty - 2015 - About Capital in the Twenty-First Century.pdf}
}

@article{smithNaturePrivilegeIntergenerational2022,
  title = {The Nature of Privilege: Intergenerational Wealth in Animal Societies},
  shorttitle = {The Nature of Privilege},
  author = {Smith, Jennifer E and {Natterson-Horowitz}, B and Alfaro, Michael E},
  editor = {Simmons, Leigh},
  year = {2022},
  month = feb,
  journal = {Behavioral Ecology},
  volume = {33},
  number = {1},
  pages = {1--6},
  issn = {1045-2249, 1465-7279},
  doi = {10.1093/beheco/arab137},
  urldate = {2024-09-11},
  abstract = {Abstract             Wealth inequality is widespread across human societies, from pastoral and small-scale agricultural groups to large modern social structures. The intergenerational transfer of wealth privileges some individuals over others through the transmission of resources external to an individual organism. Privileged access to household wealth (e.g., land, shelter, silver) positively influences the destinies of some (and their descendants) over others in human societies. Strikingly parallel phenomena exist in animal societies. Inheritance of nongenetic commodities (e.g., a nest, territory, tool) external to an individual also contributes greatly to direct fitness in animals. Here, we illustrate the evolutionary diversity of privilege and its disparity-generating effects on the evolutionary trajectories of lineages across the Tree of Life. We propose that integration of approaches used to study these patterns in humans may offer new insights into a core principle from behavioral ecology---differential access to inherited resources---and help to establish a broad, comparative framework for studying inequality in animals.},
  copyright = {https://academic.oup.com/journals/pages/open\_access/funder\_policies/chorus/standard\_publication\_model},
  langid = {english},
  file = {C:\Users\niekk\Zotero\storage\SHWLGXAD\Smith et al. - 2022 - The nature of privilege intergenerational wealth .pdf}
}

@article{soleLiquidBrainsSolid2019,
  title = {Liquid Brains, Solid Brains},
  author = {Sol{\'e}, Ricard and Moses, Melanie and Forrest, Stephanie},
  year = {2019},
  month = apr,
  journal = {Philosophical Transactions of the Royal Society B: Biological Sciences},
  volume = {374},
  number = {1774},
  pages = {20190040},
  publisher = {Royal Society},
  doi = {10.1098/rstb.2019.0040},
  urldate = {2024-09-11},
  abstract = {Cognitive networks have evolved a broad range of solutions to the problem of gathering, storing and responding to information. Some of these networks are describable as static sets of neurons linked in an adaptive web of connections. These are `solid' networks, with a well-defined and physically persistent architecture. Other systems are formed by sets of agents that exchange, store and process information but without persistent connections or move relative to each other in physical space. We refer to these networks that lack stable connections and static elements as `liquid' brains, a category that includes ant and termite colonies, immune systems and some microbiomes and slime moulds. What are the key differences between solid and liquid brains, particularly in their cognitive potential, ability to solve particular problems and environments, and information-processing strategies? To answer this question requires a new, integrative framework. This article is part of the theme issue `Liquid brains, solid brains: How distributed cognitive architectures process information'.},
  keywords = {ants,cognition,evolution,immunology,neurons,swarms},
  file = {C:\Users\niekk\Zotero\storage\MDUCQYI7\Solé et al. - 2019 - Liquid brains, solid brains.pdf}
}

@article{stopczynskiHowPhysicalProximity2018,
  title = {How {{Physical Proximity Shapes Complex Social Networks}}},
  author = {Stopczynski, Arkadiusz and Pentland, Alex `Sandy' and Lehmann, Sune},
  year = {2018},
  month = dec,
  journal = {Scientific Reports},
  volume = {8},
  number = {1},
  pages = {17722},
  issn = {2045-2322},
  doi = {10.1038/s41598-018-36116-6},
}

@article{tothInequalityRisingWhere2021a,
  title = {Inequality Is Rising Where Social Network Segregation Interacts with Urban Topology},
  author = {T{\'o}th, Gerg{\H o} and Wachs, Johannes and Di Clemente, Riccardo and Jakobi, {\'A}kos and S{\'a}gv{\'a}ri, Bence and Kert{\'e}sz, J{\'a}nos and Lengyel, Bal{\'a}zs},
  year = {2021},
  month = feb,
  journal = {Nature Communications},
  volume = {12},
  number = {1},
  pages = {1143},
  issn = {2041-1723},
  doi = {10.1038/s41467-021-21465-0},
}

@article{uganderAnatomyFacebookSocial2011a,
  title = {The {{Anatomy}} of the {{Facebook Social Graph}}},
  author = {Ugander, J. and Karrer, B. and Backstrom, L. and Marlow, Cameron A.},
  year = {2011},
  month = nov,
  journal = {ArXiv},
  urldate = {2024-09-27},
}

@article{viningHowDoesMobility2019,
  title = {How Does Mobility Help Distributed Systems Compute?},
  author = {Vining, William F. and Esponda, Fernando and Moses, Melanie E. and Forrest, Stephanie},
  year = {2019},
  month = jun,
  journal = {Philosophical Transactions of the Royal Society B: Biological Sciences},
  volume = {374},
  number = {1774},
  pages = {20180375},
  issn = {0962-8436, 1471-2970},
  doi = {10.1098/rstb.2018.0375},
  urldate = {2024-09-11},
  abstract = {Brains are composed of connected neurons that compute by transmitting signals. The neurons are generally fixed in space, but the communication patterns that enable information processing change rapidly. By contrast, other biological systems, such as ant colonies, bacterial colonies, slime moulds and immune systems, process information using agents that communicate locally while moving through physical space. We refer to systems in which agents are strongly connected and immobile as               solid               , and to systems in which agents are not hardwired to each other and can move freely as               liquid               . We ask how collective computation depends on agent movement. A liquid cellular automaton (LCA) demonstrates the effect of movement and communication locality on consensus problems. A simple mathematical model predicts how these properties of the LCA affect how quickly information propagates through the system. While solid brains allow complex network structures to move information over long distances, mobility provides an alternative way for agents to transport information when long-range connectivity is expensive or infeasible. Our results show how simple mobile agents solve global information processing tasks more effectively than similar systems that are stationary.                          This article is part of the theme issue `Liquid brains, solid brains: How distributed cognitive architectures process information'.},
  langid = {english},
  file = {C:\Users\niekk\Zotero\storage\6KX5HRJK\Vining et al. - 2019 - How does mobility help distributed systems compute.pdf}
}

@article{wattsCollectiveDynamicsSmallworld1998,
  title = {Collective Dynamics of `Small-World' Networks},
  author = {Watts, Duncan J. and Strogatz, Steven H.},
  year = {1998},
  month = jun,
  journal = {Nature},
  volume = {393},
  number = {6684},
  pages = {440--442},
  publisher = {Nature Publishing Group},
  issn = {1476-4687},
  doi = {10.1038/30918},
  urldate = {2023-03-28},
  abstract = {Networks of coupled dynamical systems have been used to model biological oscillators1,2,3,4, Josephson junction arrays5,6, excitable media7, neural networks8,9,10, spatial games11, genetic control networks12 and many other self-organizing systems. Ordinarily, the connection topology is assumed to be either completely regular or completely random. But many biological, technological and social networks lie somewhere between these two extremes. Here we explore simple models of networks that can be tuned through this middle ground: regular networks `rewired' to introduce increasing amounts of disorder. We find that these systems can be highly clustered, like regular lattices, yet have small characteristic path lengths, like random graphs. We call them `small-world' networks, by analogy with the small-world phenomenon13,14 (popularly known as six degrees of separation15). The neural network of the worm Caenorhabditis elegans, the power grid of the western United States, and the collaboration graph of film actors are shown to be small-world networks. Models of dynamical systems with small-world coupling display enhanced signal-propagation speed, computational power, and synchronizability. In particular, infectious diseases spread more easily in small-world networks than in regular lattices.},
  copyright = {1998 Macmillan Magazines Ltd.},
  langid = {english},
  keywords = {Humanities and Social Sciences,multidisciplinary,Science}
}

@article{watts1999networks,
  title={Networks, dynamics, and the small-world phenomenon},
  author={Watts, Duncan J.},
  journal={American Journal of Sociology},
  volume={105},
  number={2},
  pages={493--527},
  year={1999},
  publisher={University of Chicago Press}
}
